Verifying Data Constraint Equivalence in FinTech Systems

Data constraints are widely used in FinTech systems for monitoring data consistency and diagnosing anomalous data manipulations. However, many equivalent data constraints are created redundantly during the development cycle, slowing down the FinTech systems and causing unnecessary alerts. We present EqDAC, an efficient decision procedure to determine the data constraint equivalence. We first propose the symbolic representation for semantic encoding and then introduce two light-weighted analyses to refute and prove the equivalence, respectively, which are proved to achieve in polynomial time. We evaluate EqDAC upon 30,801 data constraints in a FinTech system. It is shown that EqDAC detects 11,538 equivalent data constraints in three hours. It also supports efficient equivalence searching with an average time cost of 1.22 seconds, enabling the system to check new data constraints upon submission.

==> ack.tex <==
\section{Acknowledgment}
The data set used in the work does not contain any Personal Identifiable Information (PII).
All the data constraints shown in the example are desensitized and encrypted.
Adequate data protection was carried out during the experiment to prevent the risk of data copy leakage, and the data set was destroyed after the experiment.
The set of the data constraints are only used for academic research, and do not represent any real business situation.
	


==> aerule.tex <==
\begin{figure}[t]
	\centering
	\[
	\inference[\textsf{AE-Axiom}]
	{		
	}
	{
		\mathcal{E}(v) = \clubsuit(\mathcal{E}, v)
	}
	\]	
	
	\[
	\inference[\textsf{AE-UDF}]
	{		
		\Phi(v) = p, \ \ \ \mathcal{E}(v) = x
	}
	{
		\Phi(f(v)) = p \times [f(x) = y], \ \ \ \mathcal{E}(f(v)) = \clubsuit(\mathcal{E}, f(v))
	}
	\]	
	
	\caption{Rules for arithmetic expressions}
	\label{rule_expression}
\end{figure}

==> aralg.tex <==
\begin{algorithm}[t]
	\SetNoFillComment
	\caption{Constructing the algebraic representation.}
	\label{alg:ar}
	\KwIn{$r$: A data constraint\;}
	\KwOut{$(\Phi, \mathcal{E})$: The environment of $r$;}
	\SetKwFunction{generateAST}{generateAST}
	\SetKwFunction{serializeByBFS}{serializeByBFS}
	\SetKwFunction{AExpr}{A-Expr}
	\SetKwFunction{Predicate}{Predicate}
	\SetKwFunction{Statement}{Statement}
	\SetKwFunction{applyAE}{applyAERule}
	\SetKwFunction{applyP}{applyPRule}
	\SetKwFunction{applyS}{applySRule}
	\SetKwFunction{normalize}{normalize}
	\SetKwFunction{removenot}{removeNotOperator}
	\SetKwFunction{removenondb}{eliminateNonDBVariable}
	$t_r \leftarrow \generateAST(r)$\;
	$AEL, NL \leftarrow \serializeByBFS(r)$\;
	$\Phi \leftarrow [n \to \bot \ | \ n \in NL]$\;
	$\mathcal{E} \leftarrow [e_a \to \bot \ | \ e_a \in AEL]$\;
	
	~\\
	\tcc{\textcolor[RGB]{0, 0, 204}{Apply rules in a bottom-up manner}}
	\ForEach{$N \in NL$} {
		\If{$N$ is \AExpr}{
			$\Phi, \mathcal{E} \leftarrow \applyAE(\Phi, \mathcal{E}, N)$\;
		}
		\If{$N$ is \Predicate}{
			$\Phi, \mathcal{E} \leftarrow \applyP(\Phi, \mathcal{E}, N)$\;
		}
		\If{$N$ is \Statement}{
			$\Phi, \mathcal{E} \leftarrow \applyS(\Phi, \mathcal{E}, N)$\;
		}
	}
	~\\
	\tcc{\textcolor[RGB]{0, 0, 204}{Normalization}}
	$p \leftarrow \removenot(\Phi(r))$\;
	$p \leftarrow \removenondb(p)$\;
	\Return{p}\;
\end{algorithm}

==> arithrule.tex <==
\vspace{-2mm}

\begin{figure}[t]
	\[
	\inference[\texttt{VAR}]
	{
		u \in \mathcal{L} \cup \mathcal{V}_d \ \ \ \ \mathbf{E}' = \mathbf{E}[u \mapsto \{u, T\}] \\
	}
	{
		\mathbf{E} \vdash_e u\leadsto \mathbf{E}'
	}
	\]
	\[
	\inference[\texttt{AE}]
	{
		A = \{(t_1 \oplus t_2, \phi_1 \land \phi_2) \ | \ (t_i, \phi_i) \in \mathbf{E}(a_i)\}\\
	}
	{
		\mathbf{E} \vdash_e a_1 \oplus a_2 \leadsto \mathbf{E}[a_1 \oplus a_2 \mapsto A]
	}
	\]
	\vspace{-4mm}
	\caption{Evaluation rules of variables and arithmetic expressions}	
	\label{rule:arithexpr}
	\vspace{-5mm}
\end{figure}

==> eqralg.tex <==
\begin{algorithm}[t]
	\SetNoFillComment
	\caption{Decision procedure for data constraint equivalence verification.}
	\label{alg:eqr}
	\KwIn{$r_1, r_2$: Two data constraints\;}
	\KwOut{Whether $r_1$ and $r_2$ are semantically equivalent.}
	\SetKwFunction{generateAST}{generateAST}
	\SetKwFunction{serializeByBFS}{serializeByBFS}
	\SetKwFunction{AExpr}{A-Expr}
	\SetKwFunction{Predicate}{Predicate}
	\SetKwFunction{Statement}{Statement}
	\SetKwFunction{applyAE}{applyAERule}
	\SetKwFunction{applyP}{applyPRule}
	\SetKwFunction{applyS}{applySRule}
	\SetKwFunction{genOrbit}{PIE}
	\SetKwFunction{constructAlgRep}{constructAlgReps}
	\SetKwFunction{constructSymRep}{constructSymReps}
	\SetKwFunction{getDBVariables}{$\pi_v$}
	\SetKwFunction{getDBFunctions}{$\pi_f$}
	\SetKwFunction{SMTSolve}{SMT-Solve}	
	$p_1, p_2 \leftarrow  \constructAlgRep(r_1, r_2)$\;
	%~\\
	%\tcc{\textcolor[RGB]{0, 0, 204}{Invariant Analysis}}
	\If{$\getDBVariables(p_1) \neq \getDBVariables(p_2)$}{
		\Return{false}\;
	}
	%~\\
	 %\tcc{\textcolor[RGB]{0, 0, 204}{Certificate Analysis}}
	\If{$ \genOrbit(p_1) =  \genOrbit(p_2)$}{ 
		\Return{true}\;
	}
	%~\\
	%\tcc{\textcolor[RGB]{0, 0, 204}{Semantic Analysis}}
	$\phi_1, \phi_2 \leftarrow  \constructSymRep(p_1, p_2)$\;
	\uIf{$\SMTSolve(\lnot (\phi_1 \leftrightarrow \phi_2))$ is \textit{UNSAT}}{
		\Return{true}\;
	}
	\Return{false}\;
\end{algorithm}

==> equivalence.tex <==
\subsection{Equivalence Relation of Representation}
\label{subsec:eqrr}
This section presents two equivalence relations for the representations defined in Section~\ref{sec:algebraic},
namely the algebraic equivalence and the symbolic equivalence.
The two equivalence relations are the criterion for determining data constraints in the decision procedure (\cref{subsec:decision}).

According to Definition~\ref{def:ar}, the algebraic representation of a data constraint actually summarizes the semantics
by a polynomial function.
Based on Definition~\ref{def:se}, two data constraints must be semantically equivalent 
if and only if the two polynomials map the same values of data variables to \textbf{0} or \textbf{1} simultaneously.
Formally, the algebraic equivalence relation is defined as follows.

\begin{definition}(\textbf{Algebraic Equivalence})
	\label{def:pae}
	Two polynomials $p_1, p_2 \in \mathcal{A}$ are algebraically equivalent, denoted by $p_1 \simeq_{\mathcal{A}} p_2$,
	if and only if they evaluate to the same value for any given interpretation.
\end{definition}

Similarly, we can define the symbolic equivalence for the symbolic representations.

\begin{definition}(\textbf{Symbolic Equivalence})
	%The symbolic representations
	$\phi_1$ and $\phi_2$ are symbolically equivalent, denoted by $\phi_1 \simeq_{\Phi} \phi_2$,
	if  and only if $\phi_1$ and $\phi_2$ are both satisfied or unsatisfied for any given interpretation.
\end{definition}

According to Theorem~\ref{thm:absemantics},
we can reduce the data constraint equivalence problem to determining the algebraic equivalence and the symbolic equivalence.
On the one hand, the algebraic representations enable us to reason the syntactic properties
and design the light-weighted reasoning to decide the algebraic equivalence efficiently for specific cases.
On the other hand, the symbolic equivalence is essentially the logical equivalence of two symbolic representations,
which can be effectively determined by an SMT solver.
In what follows, we present three analyses upon the two representations (\cref{subsec:invana}$\sim$\cref{subsec:semanana}),
which finally yield an efficient decision procedure in practice (\cref{subsec:decision}).


%Particularly,
%Theorem~\ref{thm:nae} indicates that we can conduct a light-weighted reasoning of non-equivalent data constraints by examining the algebraic equivalence invariant,
%while the symbolic equivalence inspires us to find a general solution by leveraging the SMT solver.
%Moreover, the algebraic equivalence can be determined safely if we prove the algebraic congruence.
%In what follows,
%we will present how to determine the algebraic congruence efficiently (\cref{subsec:encoding}) and fuse all the equivalence relations together to design an efficient decision procedure (\cref{subsec:decision}).


==> implementation_ICSE.tex <==
\section{Implementation and Application}
\label{sec:app}

\begin{figure}[t]
	\centering
	\includegraphics[width=0.8\linewidth]{Fig/app.pdf}
	\caption{System diagram of integrating \ToolName}
	\label{fig:app}

\end{figure}

%using the Z3 SMT solver~\cite{MouraB08}. /gang{using z3 only for one component, not as a whole}
We have implemented \ToolName\ and deployed it in company A.
%The data constraints in company A are written in \textsf{Aviator}, which is an expression evaluator for Java~\cite{aviator}.
It first generates the abstract syntax tree of a data constraint and then translates it to the symbolic representation. 
To determine the logical equivalence of symbolic representations, we leverage the Z3 SMT solver~\cite{MouraB08} to perform the SMT solving.
%\yao{maybe modify and put this part before Section 3.2 (or put it to Section 2 (ends with problems))
	%	We have problems first, and then we want to solve them.}
%\yao{then, Section 2 could be ``background and motivation''}
Using the decision procedure \ToolName, 
we can promote two typical applications of the data constraint maintenance.

\smallskip
\textbf{Data Constraint Clustering.}
%When the data reconciliation platform checks each data constraint,
In a data reconciliation platform (DR platform),
equivalent data constraints introduce unnecessary computation.
%as the evaluated results must be the same for equivalent data constraints.
To reuse the available results,
we divide data constraints into several equivalent classes as clusters,
which is shown by orange arrows in Fig.~\ref{fig:app}.
The platform lazily checks each data constraint
i.e., reuse the existing result of any equivalent data constraint in a cluster.
Besides, the clusters also guide the alert generation,
eliminating redundant alerts caused by the violation of equivalent data constraints.

%The data constraints are often supplied by different teams in the FinTech systems,
%and the lack of communication can cause the redundant submission of the equivalent data constraints.
%Therefore, we can invoke the decision procedure and omit the equivalent pair in the system, finally yielding a smaller set of data constraints.
%The consolidated set of the data constraints enables the system to avoid performing the redundant examination.
%Particularly, we can persist the intermediate results, such as the algebraic equivalence invariants and the values of the permutation-insensitive encoding,
%to avoid unnecessary computation.

\smallskip
\textbf{Data Constraint Filtering.}
As shown by purple arrows in Fig.~\ref{fig:app},
\ToolName\ examines whether a new data constraint is equivalent to an existing one upon the submission.
If not, the data constraint will be stored in the system.
Otherwise, the system lists all the equivalent ones and enables the developer to reuse the checking results.
Specifically,
we invoke \ToolName\ to decide the equivalence of each existing data constraint and the newly-submitted one.
The FinTech system can maintain fewer data constraints but still check database tables sufficiently.
%Similarly to the data constraint indexing,
%we also preserve several intermediate results of the decision procedure
% to efficiently support the data constraint filtering in different rounds.

==> language.tex <==
\section{Background and Motivation}
This section presents the background of data constraints (\cref{subsec:usage})
and the motivation of equivalence verification (\cref{subsec:edc}).
%Finally, we discuss the applications of the data constraint maintenance benefited from the decision procedure (\cref{subsec:app}).

\subsection{Data Constraints in FinTech Systems}
\label{subsec:usage}
A FinTech system usually consists of a cluster of database-backed applications, which manipulate large amounts of data in the database,
making the data records exhibit specific properties.
%reflecting the business rules of financial services~\cite{simsion2004data}.
%Specifically, the applications in a FinTech system have close interactions with each other,
%in which the data values are retrieved, processed, and finally stored in database tables.
%Therefore, the data records can exhibit specific properties,  which correspond to business rules~\cite{simsion2004data}.
To improve the system reliability, the developers of industrial FinTech systems often specify data constraints
to describe target properties,
and a data reconciliation platform~\cite{bakhtouchi2020data} examines each data constraint in the runtime.
As an example,
Fig.~\ref{subfig:motivatingEx1a}
depicts the target property of the table $t$
that the income or expense is greater than zero, and the account name is not \emph{null}.
Once a data constraint is violated, 
developers can receive detailed runtime information to guide further system diagnosis.
Generally, the data constraint checking helps the developers
discover anomalous behavior of the FinTech systems in time,
reducing system risks caused by erroneous data.


%Examining data constraints could be conducted online or offline, based on trade-offs between effectiveness and cost. 
%It is a common practice to set a schedule of examining data constraints.
%Specifically, the developers can set the time period of examination for each data constraint,
%for example, examining it every minute.



%There are two main ways to examine data constraints: \textit{online}, which examines data before writing it to the database, and \textit{offline}, which examines data after writing it to the database. 
%The offline examination is usually conducted regularly and separately to avoid competing for computation resources and interrupting with the business logic systems\gang{how to describe here?}. 

\begin{comment}
In the real-world production, developers often set a schedule of checking a data constraint,
such as performing the checking every minute.
Given a set of data constraints and a schedule,
the data reconciliation platform retrieves data records from the database and validates them against every constraint according to the schedule.
Once a data constraint is violated, the developers can receive detailed runtime information to guide further system debugging and fixing.
Generally, the scheduled checking of data constraints enables the developers to 
discover anomalous behavior of the FinTech systems in time, and further reduces system risks caused by erroneous data.
\end{comment}


\subsection{Verifying Data Constraint Equivalence}
\label{subsec:edc}
%\yao{weak flow, and a bit ``too much information'' until now}

\yao{this paragraph: many constraints; many are evolving}
In reality, many development teams continuously submit data constraints to a central data reconciliation platform.
In company A, for example, around 100 teams actively submit data constraints daily to the platform,
which contains over 20 thousand data constraints in total.
%\yao{this paragraph: they write equivalent ones, and the reasons}
%\wcp{These two paragraphs should be merged. The collaboration introduces the equivalent data constraint.
%	The first para is regarded as the background of why equivalent data constraints exist. Otherwise, the first para should be removed in the section 2.1.} 
The collaborative isolation makes the developers unaware 
of submitted data constraints
and eventually introduces the redundancy.
Moreover, developers tend to be conservative about removing constraints,
as they do not want to take the risk of missing a data error.
Finally, the accumulation of equivalent constraints can become the ``technical debt\text{''} of FinTech systems.
% (aka, the ``tech debt'')

\yao{this paragraphs: they have bad consequences, add add overhead to maintenance}
Unfortunately, equivalent data constraints are quite harmful.
First, they introduce redundant computation in the FinTech system, 
causing unnecessary resource consumption, such as CPU time, memory, and network IOs.
Second, multiple alerts are fed to the developers if equivalent data constraints are violated, 
making the diagnosis process quite verbose.
Third, all the equivalent data constraints should be updated if the table schema or the target properties are changed, 
which causes extra manual efforts~\cite{YangSYC020}.
To assist the data constraint maintenance,
we need a decision procedure to determine their semantic equivalence,
which supports filtering redundant data constraints
and reusing the checking result of equivalent ones.

%Different teams may contribute data constraints for different For FinTech systems, data constraints are contributed from different teams, 
%In the production line of the FinTech company, data constraints often come from the developers in separate teams.
%In the FinTech company A, for example, there have been over xxxx developers in xx teams submitted data constraints during the past xx years.
%The isolation between the teams and developers often makes them unaware of which data constraints have been submitted by others,
%introducing equivalent data constraints in the system.
%Equivalent data constraints are quite harmful for the long-term development of the FinTech system due to the following reasons:

%Equivalent data constraints have gradually become the \text{``}technical debt\text{''} of the FinTech system, posing a tricky problem in the maintenance.




==> preliminary.tex <==
\section{Problem Formulation}
\label{sec:preliminaries}
In this section, we present the basic terminologies, including the syntax (\cref{subsec:syntax}) and the semantics (\cref{subsec:semantics}) of data constraints,
and finally define the data constraint equivalence problem (\cref{subsec:ps}).
%First, we introduce the notion of an interpretation formally as follows.
%The assumption trivially holds in the real-world scenario, while it is important for our reasoning in Sections~\ref{sec:algebraic} and~\ref{sec:hybrid}.

%The syntax in Figure~\ref{lang-syntax} enables the developers to describe the relations of the attributes in the database tables.
%In this work, we only concern the comparison between the attributes and the literals.
%Obviously, 

\subsection{Data Constraint Syntax}
\label{subsec:syntax}
Figure~\ref{lang-syntax} summarizes the core constructs of a data constraint in a simplified abstract syntax.
The data constraint language is used for specifying the property of data values. %\wcp{omit the true and false predicates}
%We illustrate the constructs in a bottom-up style as follows:
\begin{figure}[t]
	\vspace{-3mm}
	\[
	\begin{array}{llll}
	%\textit{Program} \ \ 
	&\mathcal{R}  &:=  s+\\
	&\mathcal{S} &:= x = e  \ | \ \textbf{assert}(c) \ | \ s_1; s_2 \ | \ \textbf{ite}_s(b, s_1, s_2)\\
	%& \ | \ \textbf{if} \ (c) \ \textbf{then} \ S_1 \ \textbf{else} \ S_2\\
	&\mathcal{E} &:=  \ell \ | \ v_d \ | \ e_1 \oplus e_2\\
	&\mathcal{B}   &:= e_1 \odot e_2 \\
	&\mathcal{C} &:= b \ | \ c_1 \ \textbf{and} \ c_2 \ | \ c_1 \ \textbf{or} \ c_2 \ | \ \textbf{not} \ c \ | \ \textbf{ite}_c(b, c_1, c_2)\\
	%& \ | \ \textbf{if} \ (c) \ \textbf{then} \ c_1 \ \textbf{else} \ c_2\\
	%\textsf{A-Expr}\ \ E_a &:= v \ | \ v_1 + v_2 \ | \ v_1 - v_2 \ | \ f(v)\\	
	& \odot &:=  \ \ > \ | \ < \ | \ \geq \ | \ \leq \ | \ == \ | \ \neq\\
	& \oplus &:= \ + \ | \ - \ | \ \times \ | \ \div\\
	&\mathcal{V} &:= v_{d} \ | \ x \\
	& \mathcal{L} & :=\{\ell_i \ | \ i \geq 1 \}\\
	%\textsf{Func}\ \ F &:= f_1 \ | \ f_2 \ | \ f_3 \ | \ \cdots\\
	\end{array}
	\]
	\caption{The syntax of data constraints}
	\label{lang-syntax}
	\vspace{-5mm}
\end{figure}

\begin{itemize}[leftmargin=*]
	\item A \emph{variable} is either a data variable $v_d \in \mathcal{V}_d$ corresponding to the value of a table attribute,
	or an user-defined variable $x \in \mathcal{V}_u$ storing the value temporally.
	Due to flexible schema, both kinds of the variables can have various types.
	Without loss of generality, we consider integers and strings in our syntax.
	Particularly, the strings are over a finite alphabet.
	\item A \emph{constant} supports the developers to introduce a specific value in a data constraint for the comparison with a data variable.
	For example, a developer can label the membership tier of a user with a constant string, such as \textsf{\text{``}Platinum\text{''}}, \textsf{\text{``}Gold\text{''}}, and \textsf{\text{``}Silver\text{''}}.
	%\yao{``literal'' might be confusing: in constraints, a literal is an atom or its negation}
	\item A \emph{predicate} describes the comparison among variables and constants.
	An \emph{atomic predicate} only involves the comparison between a pair of variables or constants.
	A predicate can also indicate whether the value belongs to a set of constants,
	or consist of several sub-predicates.
	We assume that the condition of $\textbf{ite}_{c}$ is an atomic predicate comparing the data variables and constants.
	%For instance, $\textbf{ite}_{C} (\textsf{ac.fee} == 0, \ \textsf{ac.tier} \ \textbf{in} \ \{\textsf{\text{``}Platinum\text{''}}, \ \textsf{\text{``}Gold\text{''}}\}, \ \textsf{ac.tier} == \textsf{\text{``}Silver\text{''}})$
	%encodes the property that the fee is 0 for the platinum or gold users.
	\item The \emph{statements} include an assignment, an assertion examining a predicate, a sequencing, and an $\textbf{ite}_{s}$ statement.
	The condition of an $\textbf{ite}_{s}$ statement has the same form as the one in an $\textbf{ite}_{c}$ predicate.
	Finally, a \emph{data constraint} consists of a finite sequence of statements.
	All the assertions in the data constraint are expected to hold upon the given database tables.
\end{itemize}

\begin{remark}
The syntax is expressive enough to specify target properties in the real world.
In particular, it covers all the constraint patterns in \cite{florez2022retrieving}, such as value comparison, categorical values, etc.
Moreover, user-defined variables support developers to write data constraints more flexibly.
We formulate our approach upon the syntax in this work
to show its capability of reasoning data constraints in different systems~\cite{YangSYC020, florez2021empirical, florez2022retrieving}.
\end{remark}


\subsection{Data Constraint Semantics}
\label{subsec:semantics}
This section provides a formal definition of the semantics of a data constraint.

\input{semantics}

\begin{definition}(\textbf{Interpretation})
	\label{def:interpretation}
	An interpretation $I$ is a mapping which maps each data variable $v_{d}$ to a value in its domain.
\end{definition}

\begin{example}
	\label{ex:interpretation}
	For the data constraint in Figure~\ref{subfig:motivatingEx1a},
	an interpretation $I$ maps \textsf{ac.t}, \textsf{ac.in}, \textsf{ac.out}, \textsf{ac.iid}, and \textsf{ac.oid} to the values in their domains, respectively.
	Specifically, $I$ can be 
	$$I = \{\textsf{ac.t} \mapsto \textsf{`IN'}, \ \textsf{ac.in} \mapsto 10, \ \textsf{ac.out} \mapsto 0, \ \textsf{ac.iid} \mapsto 1, \ \textsf{ac.oid} \mapsto 2\}$$
\end{example}

An interpretation is essentially a projection of a database record,
which determines the values of the data variables.
A data constraint poses the restriction on data values by assertions.
Any violation reveals that the content of database tables does not exhibit the target property.

Figure~\ref{fig:semantics} defines the denotational semantics of a data constraint $r$.
We use the notation $\llbracket r \rrbracket$ to represent the semantics of $r$,
which maps an interpretation $I$ to a boolean value, 
indicating whether $r$ holds under the interpretation $I$.
Specifically, we model the values of each variable by the valuation $E$, which maps each variable to a value.
Besides, we use a pair of the valuation and a boolean value 
to describe the effect of a statement on the valuation and record whether each assertion holds in the statement, respectively.
Finally, we disregard the valuation and only preserve the boolean value for a data constraint,
as we focus on the assertions rather than the values of variables.

\subsection{Data Constraint Equivalence}
\label{subsec:ps}
Based on the denotational semantics,
we can define the semantic equivalence formally as follows.

\begin{definition}(\textbf{Semantic Equivalence})
	\label{def:se}
	Data constraints $r_1$ and $r_2$ are semantically equivalent, denoted by $r_1 \simeq r_2$, if and only if
	$\denot{r_1}(I) = \denot{r_2}(I)$ for any interpretation $I$.
\end{definition}

\begin{example}
	%Consider the data constraints in Figure~\ref{fig:motivatingEx}, 
	%which examine the five attributes of the database tables.
	%$I$ defined in Example~\ref{ex:interpretation} is a model of the data constraint in Figure~\ref{subfig:motivatingEx1a}.
	%However, $I' = I[\textsf{ac.in} \mapsto 0]$ is not a model of the data constraint, 
	%as the variable \textsf{amount} evaluates to 0, which violates the assertion.
	%Here $I'$ maps \textsf{ac.in} to 0 and other attributes in the same way of $I$.
	An interpretation $I$ is the model of $r_1$ in Figure~\ref{subfig:motivatingEx1a} and $r_2$ in Figure~\ref{subfig:motivatingEx1b}
	as long as it maps \textsf{ac.t}, \textsf{ac.in}, \textsf{ac.out}, \textsf{ac.iid}, and \textsf{ac.oid} to $\textsf{t}$, $\textsf{in}$, $\textsf{out}$, $\textsf{iid}$, and $\textsf{oid}$, respectively, such that
	\begin{equation*}
	\label{eq:ex}
	((\textsf{t} = \textsf{`IN'} \land \textsf{in} > 0) \lor (\textsf{t} \neq \textsf{`IN'} \land \textsf{out} > 0))
	\land \textsf{iid} \neq \textbf{nil} \land \textsf{oid} \neq \textbf{nil}
	\end{equation*}
	is satisfied. 
	%Similarly, each interpretation makes the assertions of the data constraint $r_2$ hold in Figure~\ref{subfig:motivatingEx1b} if and only if it makes Equation~\ref{eq:ex} satisfied.
	Therefore, $r_1$ and $r_2$ are semantically equivalent.
\end{example}

The semantic equivalence shows that the data constraints depict the same property of data values.
Finally, we can formalize the data constraint equivalence problem as follows.
%The values of the attributes in the database tables exhibit the property described by the data constraints,
%which indicates the expected effect of the database-backed applications.
%According to the definition of semantic equivalence, we can finally formalize 

\begin{definition}(\textbf{Data Constraint Equivalence Problem})
	\label{def:problem}
	Given two data constraints $r_1$ and $r_2$ in the syntax shown in Figure~\ref{lang-syntax},
	determine whether or not $r_1$ is semantically equivalent to $r_2$.
\end{definition}

Solving the data constraint equivalence problem is key to effective data constraint maintenance,
%supporting various applications of data constraints.
Unfortunately, it is quite difficult to find an efficient solution to the problem.
Formally, we state the theorem to demonstrate the complexity barrier of the problem.
%\footnote{The proofs of the theorems in the paper are provided in the supplementary material.}.
%and prove it in the supplementary material.
%\wcp{Move the decidability at the end of the approach.}
%In the real-world scenario, we often need to remove the equivalent data constraints, which are redundant and unnecessary to examine, from a set of data constraints.
%Besides, it is also necessary to filter a newly-submitted data constraint if it is semantically equivalent to an existing one.
%We discuss the two applications, namely data constraint consolidation and filtering, in Section~\ref{sec:impl} in detail and evaluate them in Section~\ref{sec:eval}.

%\yao{perhaps a bit early?}
\begin{theorem}(\textbf{Complexity Barrier})
	\label{thm:decomp}
	Data constraint equivalence problem is NP-hard.
\end{theorem}

\textbf{Roadmap.}
To determine the semantic equivalence,
we propose two novel representations to abstract the data constraint semantics (\cref{sec:algebraic}),
namely the algebraic representation (\cref{subsec:algebraic_construction}) and the symbolic representation (\cref{subsec:symbolic_construction}),
based on which we design an efficient decision procedure (\cref{sec:hybrid}).
Particularly, we achieve the equivalence verification in polynomial time via reasoning the algebraic representations (\cref{subsec:invana}$\sim$\cref{subsec:encoding}),
which is our main technical contribution.
To assure completeness,
we also establish the equivalence verification upon the symbolic representations (\cref{subsec:semanana}).
By fusing the analyses upon two representations as a whole (\cref{subsec:decision}),
our decision procedure \ToolName\ achieves high efficiency in practice and also features the soundness and completeness theoretically.

==> prule.tex <==
\begin{figure}
	%\begin{subfigure}[b]{0.47\textwidth}
	%\[
	%\inference[\textsf{P-TRUE}]
	%{		
%		\mathbf{S}' = \mathbf{S}[\mathbf{true} \mapsto \mathbf{1}]
	%}
	%{
	%	\mathbf{E}, \mathbf{S} \vdash_c \textbf{true} \rightsquigarrow \mathbf{E}, \mathbf{S}'
	%}
	%\]	
	%\end{subfigure}
	%\begin{subfigure}[b]{0.47\textwidth}
	%\[
	%\inference[\textsf{P-FALSE}]
	%{		
%		\mathbf{S}' = \mathbf{S}[\mathbf{false} \mapsto \mathbf{0}]
	%}
	%{
%		\mathbf{E}, \mathbf{S} \vdash_c \textbf{false} \rightsquigarrow \mathbf{E}, \mathbf{S}'
	%}
	%\]	
	%\end{subfigure}
	\[
	\inference[\textsf{P-VarCmp}]
	{	
		\{(u_1^{(i)}, p_1^{(i)})\}_{i = 0}^{n_1} = \mathbf{E}(v_1), \ \ \ \{(u_2^{(j)}, p_2^{(j)})\}_{j = 0}^{n_2}= \mathbf{E}(v_2)\\
		p = \sum_{i = 1}^{n_1} \sum_{j = 1}^{n_2} [u_1^{(i)} \odot u_2^{(j)}] \times p_1^{(i)} \times p_2^{(j)}, \ \ \ 
		\mathbf{S}' = \mathbf{S}[v_1 \odot v_2 \mapsto p]  
	}
	{
		\mathbf{E}, \mathbf{S} \vdash_c v_1 \odot v_2 \rightsquigarrow \mathbf{E}, \mathbf{S}'
	}
	\]	
	\[
	\inference[\textsf{P-VarLitCmp}]
	{		
		\{(u^{(i)}, p^{(i)})\}_{i = 0}^{n} = \mathbf{E}(v), \ \ \ 
		\mathbf{S}' = \mathbf{S}[v \odot \ell \mapsto \sum_{i = 0}^{n} [u^{(i)} \odot \ell] \times p^{(i)}]  
	}
	{
		\mathbf{E}, \mathbf{S} \vdash_c v \odot \ell \rightsquigarrow \mathbf{E}, \mathbf{S}'
	}
	\]	
	\[
	\inference[\textsf{P-VarInSet}]
	{		
		\{(u^{(i)}, p^{(i)})\}_{i = 0}^{n} = \mathbf{E}(v), \ \ \ 
		\mathbf{S}' = \mathbf{S}[v \ \textbf{in} \  L \mapsto \sum_{i = 0}^{n} (\sum_L u^{(i)}) \times p^{(i)}]
	}
	{
		\mathbf{E}, \mathbf{S} \vdash_c v \ \textbf{in} \  L  \rightsquigarrow \mathbf{E}, \mathbf{S}'
	}
	\]	
	\begin{subfigure}[b]{0.47\textwidth}
	\[
	\inference[\textsf{P-AND}]
	{		
		\mathbf{S}'  = [c_1 \ \textbf{and} \ c_2 \mapsto \mathbf{S}(c_1) \times \mathbf{S}(c_2)]
	}
	{
		\mathbf{E}, \mathbf{S} \vdash_c c_1 \ \textbf{and} \ c_2  \rightsquigarrow \mathbf{E}, \mathbf{S}'
	}
	\]	
	\end{subfigure}
	\begin{subfigure}[b]{0.47\textwidth}
	\[
	\inference[\textsf{P-OR}]
	{		
		\mathbf{S}'  = [c_1 \ \textbf{or} \ c_2 \mapsto \mathbf{S}(c_1) + \mathbf{S}(c_2)]
	}
	{
		\mathbf{E}, \mathbf{S} \vdash_c c_1 \ \textbf{or}\ c_2  \rightsquigarrow \mathbf{E}, \mathbf{S}'
	}
	\]	
	\end{subfigure}
	
	\vspace{1.5mm}
	
\begin{subfigure}[b]{0.3\textwidth}
\[
\inference[\textsf{P-NOT}]
{		
	\mathbf{S}'  = [\textbf{not} \ c \mapsto not(\mathbf{S}(c))]
}
{
	\mathbf{E}, \mathbf{S} \vdash_c \textbf{not} \ c  \rightsquigarrow \mathbf{E}, \mathbf{S}'
}
\]	
\end{subfigure}
	\begin{subfigure}[b]{0.69\textwidth}
	\[
	\inference[\textsf{P-ITE}]
	{		
		p = \mathbf{S}(b), \ \ \ p_1 = \mathbf{S}(c_1), \ \ \ p_2 = \mathbf{S}(c_2)\\
		\mathbf{S}'  = [\textbf{ite}_c(b, c_1, c_2) \mapsto p \times p_1 + not(p) \times p_2]
	}
	{
		\mathbf{E}, \mathbf{S} \vdash_c \textbf{ite}_c(b, c_1, c_2) \rightsquigarrow \mathbf{E}, \mathbf{S}'
	}
	\]
	\end{subfigure}
	\vspace{1mm}
	\caption{Rules for evaluating predicates}
	\label{rule_predicate}
	\vspace{-4mm}
\end{figure}

==> srrule.tex <==
\begin{figure}[t]
	\centering
	\vspace{-2mm}
	\begin{subfigure}[b]{0.49\linewidth}
		\centering
		\[
		\inference[\textsf{F-LitM}]
		{		
		}
		{
			[x \odot \ell] \vdash_f (\widetilde{\kappa}(x) \odot \kappa(\ell))
		}
		\]
	\end{subfigure}
	\hfill
	\begin{subfigure}[b]{0.49\linewidth}
	\centering
	\[
	\inference[\textsf{F-VarM}]
	{		
	}
	{
		[x \odot y] \vdash_f (\widetilde{\kappa}(x) \odot \widetilde{\kappa}(y))
	}
	\]	
	\end{subfigure}
	%\begin{subfigure}[b]{0.3\linewidth}
	%	\centering
	%	\[
	%	\inference[\textsf{H-Zero}]
	%	{		
	%		p = \textbf{0}
	%	}
	%	{
	%		\sigma(p) = \lambda(\mu(\textbf{0})) 
	%	}
	%	\]	
	%\end{subfigure}
	%\hfill
	%\vspace{3mm}
	%\begin{subfigure}[b]{0.3\linewidth}
	%	\centering
	%	\[
	%	\inference[\textsf{H-One}]
	%	{		
	%		p = \textbf{1}
	%	}
	%	{
	%		\sigma(p) = \lambda(\mu(\textbf{1})) 
	%	}
	%	\]	
	%\end{subfigure}
	\begin{subfigure}[b]{0.49\linewidth}
		\centering
		\[
		\inference[\textsf{F-SumP}]
		{		
			p=\sum_{i=1}^{n} p_i, \ \ \ \ \forall 1 \leq i \leq n, \ p_i \vdash_f \phi_i
		}
		{
			p \vdash_f \bigvee_{i = 1}^{n} \phi_i
		}
		\]	
	\end{subfigure}
	\hfill
	\begin{subfigure}[b]{0.49\linewidth}
		\centering
		\[
		\inference[\textsf{F-ProdP}]
		{		
			p = \prod_{i = 1}^{n} p_i,  \ \ \ \ \forall 1 \leq i \leq n, \ p_i \vdash_f \phi_i
		}
		{
			p \vdash_f \bigwedge_{i = 1}^{n} \phi_i
		}
		\]	
	\end{subfigure}
	\caption{Rules of constructing the symbolic representation}
	\label{fig:srrule}
	\vspace{-4mm}
\end{figure}

==> srule.tex <==
\begin{figure}[t]  
	\begin{subfigure}[b]{0.49\textwidth}
	\[
	\inference[\textsf{S-AssDV}]
	{		
		\mathbf{E}' = \mathbf{E}[x \mapsto \{(v_d, \textbf{1})\}]
	}
	{
		p, \mathbf{E}, \mathbf{S} \vdash_s x = v_d \rightsquigarrow p, \mathbf{E}', \mathbf{S}
	}
	\]
	\end{subfigure}
	\begin{subfigure}[b]{0.49\textwidth}
	\[
	\inference[\textsf{S-AssLit}]
	{		
		\mathbf{E}' = \mathbf{E}[x \mapsto \{(\ell, \textbf{1})\}]
	}
	{
		p, \mathbf{E}, \mathbf{S} \vdash_s x = \ell \rightsquigarrow p, \mathbf{E}', \mathbf{S}
	}
	\]	
	\end{subfigure}
	\[
	\inference[\textsf{S-Assert}]
	{		
		\mathbf{E}, \mathbf{S} \vdash_c c \rightsquigarrow \mathbf{E}', \mathbf{S}', \ \ \ 
		p_1 = \mathbf{S}'(c),  \ \ \ 
		p' = p \times p_1
	}
	{
		p, \mathbf{E}, \mathbf{S} \vdash_s \textbf{assert}(c) \rightsquigarrow p', \mathbf{E}', \mathbf{S}'
	}
	\]
	\[
	\inference[\textsf{S-Seq}]
	{		
		p, \mathbf{E}, \mathbf{S} \vdash_s s_1 \rightsquigarrow p_1, \mathbf{E}_1, \mathbf{S}_1, \ \ \ 
		p_1, \mathbf{E}_1, \mathbf{S}_1 \vdash_s s_2 \rightsquigarrow p', \mathbf{E}', \mathbf{S}'
	}
	{
		p, \mathbf{E}, \mathbf{S} \vdash_s s_1; s_2 \rightsquigarrow p', \mathbf{E}', \mathbf{S}'
	}
	\]
	
	\[
	\inference[\textsf{S-ITE}]
	{		
		\mathbf{E}, \mathbf{S} \vdash_c c \rightsquigarrow \mathbf{E}', \mathbf{S}', \ \ \
		p_1 = p \times \mathbf{S}'(b), \ \ \ p_2 = p \times not(\mathbf{S}'(b))\\
		p_1, \mathbf{E}', \mathbf{S}' \vdash_s s_1 \rightsquigarrow p \times \mathbf{S}'(b) \times p'_1, \mathbf{E}_1', \mathbf{S}_1', \ \ \ 
		p_2, \mathbf{E}', \mathbf{S}' \vdash_s s_2 \rightsquigarrow p \times not(\mathbf{S}'(b)) \times p'_2, \mathbf{E}_2', \mathbf{S}_2'
	}
	{
		p, \mathbf{E}, \mathbf{S} \vdash_s \textbf{ite}_s(b, s_1, s_2) \rightsquigarrow p \times (\mathbf{S}'(b) \times p'_1 + not(\mathbf{S}'(b)) \times p'_2), \ \mathbf{E}_1' \uplus_{\mathbf{E}} \mathbf{E}_2', \ \mathbf{S}_1' \uplus_{\mathbf{S}} \mathbf{S}_2'
	}
	\]
	
	\caption{Rules for evaluating statements}
	\label{rule_statement}
	\vspace{-3mm}
\end{figure}
